Federated Feature Selection for Cyber-Physical Systems of Systems

Autonomous vehicles (AVs) generate a massive amount of multi-modal data that once collected and processed through Machine Learning algorithms, enable AI-based services at the Edge. In fact, not all these data contain valuable, and informative content but only a subset of the relative attributes should be exploited at the Edge. Therefore, enabling AVs to locally extract such a subset is of utmost importance to limit computation and communication workloads. Achieving a consistent subset of data in a distributed manner imposes the AVs to cooperate in finding an agreement on what attributes should be sent to the Edge. In this work, we address such a problem by proposing a federated feature selection algorithm where all the AVs collaborate to filter out, iteratively, the redundant or irrelevant attributes in a distributed manner, without any exchange of raw data. This solution builds on two components: a Mutual-Information-based feature selection algorithm run by the AVs and a novel aggregation function based on the Bayes theorem executed on the Edge. Our federated feature selection algorithm provably converges to a solution in a finite number of steps. Such an algorithm has been tested on two reference datasets: MAV with images and inertial measurements of a monitored vehicle, WESAD with a collection of samples from biophysical sensors to monitor a relative passenger. The numerical results show that the fleet finds a consensus with both the datasets on the minimum achievable subset of features, i.e., 24 out of 2166 (99\%) in MAV and 4 out of 8 (50\%) in WESAD, preserving the informative content of data.

==> sections/model.tex <==
\section{System assumptions}
\label{sec:problem_statement}
%\added[id=PC]{i metodi basati su MI vanno bene perche' le features in applicazioni IoT sono segnali che vengono digitalizzati e quantizati quindi descritti attreverso variabili intere }
In this section we describe the reference scenario and the system assumptions considered in this paper, as shown in Figure \ref{fig:sys_arch}.  
We consider a scenario where a set of \acp{AV}, implementing an \ac{ADS} each, collect data generated by the sensors integrated in a \ac{CPSoS} and collaborate with the others \acp{ADS} to learn the minimal, and most informative, set of features from their local dataset. To this end, \acp{AV} execute an in-network data filtering process through our \ac{FFS} approach. In this phase, \acp{AV} exchange with each others  control information in order to reach a consensus to identify the most informative feature set. Finally, the globally shared feature set is \replaced[id=PC]{used}{use} as compression scheme before starting the transmission of data to the \ac{ES}. Note that, in this system the \acp{AV} are only responsible for finding, in a collaborative way, the best compression scheme applicable to the their local data, based only on the control information they exchange with each others. Moreover, the \ac{ES} has a three-fold role: i) it \replaced[id=PC]{acts}{act} as central coordinating entity in the \ac{FFS} process whose purpose is to aggregate the partial control information sent by the \acp{AV}; ii) it acts as final collector for the compressed data, once the \ac{FFS} is completed and, iii) runs the \ac{AI} algorithm to extract knowledge from data. 
% The final feat compression scheme for limiting the amount of data transmitted to \ac{ES} without degrading its informative content. 
% Two different learning tasks are assumed 
To validate the performance of the proposed \ac{FFS} method we target two different user cases. The first one refers to the localization of  an  AV  in the  environment based on images and inertial measurements, and the second one regards the physiological-state monitoring in the automotive domain. 
We define two different sub-systems part of the same \ac{CPSoS}: the \ac{ADS} of above, and an \ac{HSMS} to learn the feeling perceived from a passenger relatively to the \ac{ADS} driving style. Therefore, we assume each \ac{AV} to be equipped with a camera to capture images from the surrounding environment aside some inertial sensors, for the former learning task, and a set of body sensors, such as, \ac{ECG}, \ac{EDA}, \ac{EMG}, and \ac{RSP} for the latter task. 
% Finally, a suitable radio medium, like IEEE 802.11p or Cellular-V2X (C-V2X) \cite{8746562,vukadinovic20183gpp}, is assumed to transmit the features to an \ac{ES}, where the learning tasks are performed. 
Each \ac{AV} is able to locally synchronize the multi-sensory data such that, for each image, it is possible to associate the corresponding inertial measurements leading to an \emph{enhanced Raw Input Datum} (eRID). Moreover, we assume that, according to the scenario at hand, each \ac{AV} is able to associate a label to the collected data, e.g., a GPS location, relative positioning, or a feedback by the user, or any other information that can be added to the data and used only for training the \ac{ML} model. Note that for the scope of this paper it is not important the specific semantic of the labelling, but it is enough to assume a labelling process. \acp{AV} are also equipped with a relatively small edge computing unit (e.g., a RaspeberryPi or, at most, an Nvidia Jetson Nano) able to cache data and \replaced[id=PC]{execute}{executing} the feature selection task, before starting the data transmission. Additionally, \acp{AV} are endowed with a radio communication interface to communicate toward the \ac{ES}. It must be noted that the task is not collecting images of the environment, or physiological parameters of the user but, conversely, retrieving the information associated to those images or to those physiological sensors, e,g., the position of the \ac{AV} with respect to the surrounding or the user mood. In particular, the latter is labelled according to the classification scale provided by questionnaires like PANAS, SSSQ or SAM \cite{Schmidt2018}, which associates numerical labels to the physiological states. 
%expressed by a number of integer values ranging from $4$ to $9$.
%We remark that the need for labelling has to be used in the training phase only, as in every supervised learning task, which is mandatory to map an input to an output based on example input-output pairs \cite{russell2010artificial}. 
% Finaly, the architecture implements an in-network computational paradigm where \acp{AV} collectively execute the \ac{FFS} for pre-filtering the collected data in order to identify the most informative attributes, i.e., features. In our system the selected features are used as a data compression scheme to save communication resource during the data collection process towards the \ac{ES}.  
% Finally, the deployed architecture implements an in-network computational paradigm, where \acp{AV}  pre-filter the collected information through our \ac{FFS} approach. The compressed data is transmitted by  to the \ac{ES} for further  
% The filtered data . and eventually a quantization or a data compression to further reduce the data footprint, while learning process is performed on a dense Edge Server. 
% Backing to the previous example, this means that no image is moved to the Edge if not necessary for the mission of the autonomous system itself.

\begin{figure}[tb]
\centering
    \includegraphics[width=1\columnwidth,trim={130 60 100 0},clip]{figure/CPSoS.png}
\caption{\hl{Remove MEC}}System architecture. Data sources characterize two different \acp{CPS}: the former that monitors the user through wearable sensors, the latter relative to the \ac{ADS}.}
\label{fig:sys_arch}
\end{figure}

\section{Feature selection}
\label{sec:FE_theory_MAIN}
In this section, we provide the theoretical background of the \ac{MI}-based feature selection problem and its algorithmic solution based on the \ac{CE} method.

\subsection{Background knowledge on Mutual Information}
\label{sec:FE_theory}

The \ac{FS} problem can be formally stated as follows: 
\begin{Def}[\ac{FS} Problem]
Given the input data matrix $\mathbf{X}$ composed by $n$ samples of $m$ features ($\mathbf{X} \in \mathbb{R}^{n \times m}$), and the target attributes' (or labels) vector $\mathbf{y} \in \mathbb{R}^{n}$, the feature selection problem is to find a $k$-dimensional subset $\mathbf{K} \subseteq \mathbf{X}$ with $k \leq m$, by which we can characterize $\mathbf{y}$.
\end{Def}
%Note that, both features and class label values, or just one of the two, can be quantized so as to have integer values.

Now let's start providing the necessary background knowledge on \ac{MI} that we use to measure the amount of information obtained about the class attribute through the set of selected features.
The  \ac{MI} between random variables $\mathbf{A}$ and $\mathbf{B}$ is symmetric and non-negative, and it is strictly related to the entropy $\mathbf{H}(\cdot)$, which defines the amount of information held by the variables.\added[id=PC]{ More information means greater unpredictability of the random variable, so} the entropy $\mathbf{H}(\mathbf{A})$ increases if the probability of $\mathbf{A}$ \replaced[id=PC]{decreases}{is small}, otherwise the entropy decreases.

Hence, we can assert that the entropy measures the diversity of $\mathbf{A}$ in terms of the uncertainty of its outcomes. \ac{MI} between random variables can be defined as \cite{eliece77, cover91}: 

\begin{equation} 
  \label{MI_3}
  \mathbf{I}(\mathbf{U};\mathbf{y})=\mathbf{H}(\mathbf{y})-\mathbf{H}(\mathbf{y}|\mathbf{U}),
\end{equation}

where $\mathbf{U}=\{\mathbf{x}_1 \cdots \mathbf{x}_k \; | \; k\leq m\} \subseteq \mathbf{X}  $, and $\mathbf{H}(\mathbf{y}|\mathbf{U})$ is the conditional entropy which measures the amount of information needed to describe $\mathbf{y}$, conditioned by the information carried by $\mathbf{U}$. Hence, $ \mathbf{I} (\mathbf{U};\mathbf{y})$ represents the dependence between $\mathbf{U}$ and $\mathbf{y}$, i.e., the greatest is the value $\mathbf{I}$, the greatest is the information carried by $\mathbf{U}$ on $\mathbf{y}$. 
The features selected in $\mathbf{U}$ are \acp{EA}, also known as Markov Blanket~\cite{brown09,Brown2012}. So, if the features in $\mathbf{U}$ are EAs, then the equation (\ref{MI_3}) gets its maximum.
The above considerations, and the Theorem \ref{theorem dependence of y} stated in the following provide the basis to develop our \ac{FS} algorithm, whose rigorous proof is addressed in \cite{eliece77, cover91}. 
 
 \begin{Theo} \label{theorem dependence of y}
   If the \ac{MI} between $\mathbf{U}$ and $\mathbf{y}$ is equal to the entropy of $\mathbf{y}$, then $\mathbf{y}$ is function of $\mathbf{U}$.
 \end{Theo}

In Equation (\ref{Native Optimization Porblem}) we define the optimization problem that, if solved it would provide the optimal global solution for the \ac{FS} problem. 
\begin{gather} 
\label{Native Optimization Porblem}
\displaystyle \mbox{arg}\max_{\mathbf{U}} \mathbf{I}(\mathbf{U};\mathbf{y}) \\
\nonumber
\mathbf{U}=\{\mathbf{x}_1 \cdots \mathbf{x}_k \; | \; k\leq m\} \subseteq \mathbf{X}
\end{gather}%
Since the optimal solution $\mathbf{U}$ is found among all combinations of feature indices of the native set $\mathbf{X}$, this is an Integer Programming (IP) optimization problem that is NP-hard \cite{Chaovalitwongse2009}. 

A way to make it computationally tractable, is to approach it through an iterative algorithm which selects and adds to the subset $\mathbf{U}$ one feature at a time as defined in Equation~\ref{Incremental Optimization Porblem}
\begin{gather} 
\label{Incremental Optimization Porblem}
\displaystyle \mbox{arg}\max_{\mathbf{x}_j \in \mathbf{X}\setminus\mathbf{U}} \mathbf{I}(\mathbf{x}_j;\mathbf{y}|\mathbf{U}), \\
\nonumber
\mathbf{U}=\{\mathbf{x}_1 \cdots \mathbf{x}_{k-1} \; | \; k\leq m\} \subseteq \mathbf{X}.
\end{gather}
The main drawback of this algorithm is that it might end up with a sub-optimal solution because selecting the features one by one the algorithm makes the implicit assumption that they are independent, which might not hold true. Theoretical foundations for the incremental version of the feature selection algorithms has been proven by the authors in \cite{cover91, eliece77}.
% , whose main results are shown in the equations (\ref{MI property 3}), and (\ref{joined MI}).
%
% \begin{gather}
% \label{MI property 3}
% \mathbf{I}(\mathbf{U};\mathbf{y})=\mathbf{I}(\mathbf{x}_1\cdots \mathbf{x}_k;\mathbf{y})=\displaystyle \sum_{j=1}^{k} \mathbf{I}(\mathbf{x}_j;\mathbf{y}|\mathbf{x}_{j-1}\cdots \mathbf{x}_1)\\
% \nonumber
% \mathbf{U}_{k-1} \cup \mathbf{x}_k=\mathbf{U}_{k}\\
% \label{joined MI}
% \mathbf{I}(\mathbf{U}_{k};\mathbf{y})= \mathbf{I}(\mathbf{U}_{k-1};\mathbf{y})+\mathbf{I}(\mathbf{x}_k;\mathbf{y}|\mathbf{U}_{k-1}).
% \end{gather}
%
% In order to provide a global solution to prob In this paper we relax the independence assumption among features and exploiting from Equations (\ref{MI property 3}) and (\ref{joined MI}) we 

% allow to select, iteratively, the features in $\mathbf{U}$, so that \ac{MI} can be maximized. Precisely, in the first step the j'-th feature $\mathbf{x}_{j'} \;|\; 1 \leq j' \leq m$ is selected from the native set $\mathbf{X}$, so that it shares the largest \ac{MI} with the class attribute $\mathbf{y}$. In the next iterations, a feature $\mathbf{x}_j$ is selected if it contributes in achieving the maximum of \ac{MI} jointly with the already selected features.
%$\{\mathbf{x}_1 \cdots \mathbf{x_{j-1}}\} \;|\;j=1 \cdots k \leq m$, the new features to add are chosen in the native set minus the features already selected.
% Hence, the incremental optimization problem can be stated as follows: 
% \begin{gather} 
% \label{Incremental Optimization Porblem}
% \displaystyle \mbox{arg}\max_{\mathbf{x}_j \in \mathbf{X}\setminus\mathbf{U}} \mathbf{I}(\mathbf{x}_j;\mathbf{y}|\mathbf{U}), \\
% \nonumber
% \mathbf{U}=\{\mathbf{x}_1 \cdots \mathbf{x}_{k-1} \; | \; k\leq m\} \subseteq \mathbf{X}.
% \end{gather}
%
Another issue in dealing with the optimization problem in (\ref{Native Optimization Porblem})-(\ref{Incremental Optimization Porblem}) is how  efficiently evaluating both the entropy and \ac{MI} even for datasets with a small number of samples. This problem can be overcome, by using the powerful numerical tool MIToolbox \cite{Brown2012}.  

Before dealing with a numerically tractable solution of the problem in equations (\ref{Native Optimization Porblem})-(\ref{Incremental Optimization Porblem}), we want to provide an intuitive proof based on the relation between \ac{MI} and the entropy. Considering the example in Figure \ref{figure_example}, the circles are the entropy of the random variables $\mathbf{A},\textbf{B},\mathbf{U},\mathbf{y}$, and the gray regions are the information carried by the variable $\mathbf{A}(\mathbf{B})$ on $\mathbf{y}$. The dashed area shows the information redundancy of the variable  $\mathbf{A}(\mathbf{B})$  given the already selected variables in $\mathbf{U}_{j-1}$. In this example, the variable $\mathbf{A}$ is the one that should be added to the set $\mathbf{U}$ because it is more informative  than $\mathbf{B}$ on  $\mathbf{y}$ , i.e., its grey area is larger than the one of $\mathbf{B}$, and it is less redundant than $\mathbf{B}$ w.r.t. to $\mathbf{U_{j-1}}$.

\begin{figure}[ht]
\begin{center}
  \includegraphics[width=1\columnwidth,trim={0 0 0 0},clip]{figure/example.eps}
  \caption{Example of the relationship between Mutual Information and Entropy} \label{figure_example} 
 \end{center}
 \end{figure}
\subsection{CE-based feature selection based algorithm}
In this section, we provide an algorithm that in a finite number of steps is able to find a solution that well approximates \replaced[id=PC]{ the one found}{that found} by solving Problem (\ref{Native Optimization Porblem}) making negligible the assumption of independence among features introduced in Problem (\ref{Incremental Optimization Porblem}). This means that, instead of selecting one \ac{EA} at a time, we can select a set of \acp{EA} jointly. 

Our algorithm is based on the following condition: if the set $\mathbf{U}$ contains only \acp{EA}, then $\mathbf{I}(\mathbf{U}; \mathbf{y}) \rightarrow \mathbf{H}(\mathbf{y} )$, which implies that $\mathbf{H}( \mathbf{y}| \mathbf{U}) \rightarrow 0$~\cite{cover91, eliece77}. 
 Note that with our approach, we avoid the greedy research of the set $\mathbf{U}$, among  all the possible  $\binom{m}{k}$ solutions, which realizes $\mathbf{H}( \mathbf{y}| \mathbf{U}) \rightarrow 0$ .
To this end, we adopt the stochastic research of the solution. The idea behind the proposed approach is to associate the $i$-th feature, with $i=1,\cdots,m$, to a binary variable $z_i\sim \mathrm{Bernoulli}(p_i)$. Our algorithm finds the variables  $z_i, \: i=1,\cdots,m$ that must have $p_i \rightarrow 1$, so that the objective function $\mathcal{O}(\mathbf{U}(\mathbf{z}))$ given by $\mathbf{H}( \mathbf{y}| \mathbf{U})$ is close to $0$. This is called \ac{ASP}  \cite{rubinstein04}. In this way, we get the optimal distribution of the binary vector $\mathbf{z}$ through which we identify the features to select, i.e. the $i$-th feature is selected if $p_i \rightarrow 1$. It is worth noting that  searching the solution of the optimization problem through the definition of the \ac{ASP} has the advantage to address the native  problem in equations (\ref{Native Optimization Porblem}) as convex problem.\footnote{More details are in Section 4 of \cite{rubinstein04}.} 

We can formulate the \ac{ASP} as a minimization problem, as shown in the following. 
% The last step in defining our \ac{ASP} is to assume that $z_1 \cdots z_m$ are independent Bernoulli random variables where the probabilities to be selected, i.e  $z_i\rightarrow 1 \;i=1\cdots m$, are $p_1 \cdots p_m$, respectively. 
Briefly, we need to find the probability distribution $g(\mathbf{z},\mathbf{p})$ of the values in $\mathbf{z}$ equal to $1$ that solves the equation: %$P_v(\mathcal{O}(\mathbf{U}(\mathbf{z})) \leq \gamma)$ where  $\gamma$ is the minimum value that the objective function can assume for given set of selected features. 

%This problem becomes our \textbf{\emph{DISR}}. 
%Note that, $P_v(\mathcal{O}(\mathbf{U}(\mathbf{z}))\geq \gamma)$ can be estimated through the following equation given the probability distribution function $g(\mathbf{z},v)$: 

\begin{equation} 
  \label{probability estimation}
         P_{\mathbf{p}}(\mathcal{O}(\mathbf{U}(\mathbf{z}))\leq \gamma)=\sum_{\{\mathbf{z}\}}\mathcal{I}_{\{\mathcal{O}(\mathbf{U}(\mathbf{z}))\leq \gamma\}} \:g(\mathbf{z},\mathbf{p})
 \end{equation}%
where  $\mathcal{I}_{\{\cdot\}} $ is the indicator function of the event $\mathcal{O}(\mathbf{U}(\mathbf{z}))\leq \gamma$, and $ \gamma$ is the minimum value for our objective function. Precisely, $\gamma$ at step t is calculated as the percentile $1-\beta$ of the objective function calculated \added[id=PC]{by} using the samples drawn from the distribution $g(\mathbf{z},\mathbf{p})$ at step t. Note that, the authors in \cite{rubinstein04} recommend to set $\beta$ in the range $0.9-0.95$ 

The indicator function is equal to $1$ for all the possible configurations in $\mathbf{z}$ that  verify the event $\mathcal{O}(\mathbf{U}(\mathbf{z}))\leq \gamma$, and $0$ otherwise.

A well known approach to estimate $g(\mathbf{z},\mathbf{p})$ is to use the Likelihood Ratio (LR) estimator with reference parameter $\mathbf{p}$. The optimal value $\mathbf{p}^*$ for the distribution can be calculated from the theory of LR estimation \cite{rubinstein04} through the following equation:
\begin{equation} 
  \label{parameter estimation}
         \mathbf{p}^*=\displaystyle arg\min_{\mathbf{p}} \frac{1}{S} \sum_{j=1}^{S}\mathcal{I}_{\{\mathcal{O}(\mathbf{U}(\mathbf{z}_j))\leq \gamma\}} \:\mbox{ln}(g(\mathbf{z}_j,\mathbf{p}))
 \end{equation}%
where $\mathbf{Z}=\{\mathbf{z}_1, \cdots, \mathbf{z}_S\}$ is a set of possible  samples drawn from the distribution $g(\mathbf{z},\mathbf{p})$.

As stated above $\mathbf{z}_j=[z_{1j} \cdots z_{mj} ]$ is a vector of independent Bernoulli random variables where $z_{ij}$ takes value equal to $1$ with probability $p_{i}$ and $0$ with probability $1-p_{i}$. 
%Then for the assumptions stated above, 
Hence, $g(\mathbf{z}_j,\mathbf{p})$ 
%of the ones in $\mathbf{z}$ can be rewritten with parameter $v=\mathbf{p}=[p_{1} \cdots p_{m}]$ as in the following:
can be written as:

\begin{equation} 
  \label{pdf}
                           g(\mathbf{z}_j,\mathbf{p})=\displaystyle \prod_{i=1}^m p_i^{z_{ij}}(1-p_i)^{(1-z_{ij})} \: ; \: z_{ij} \in \{0,1\}
 \end{equation}
 
Given that objective function in equation (\ref{parameter estimation}) is concave \footnote{The logarithm is a concave function, the indicator function is $0$ or $1$ so the weighted sum of concave functions gives still a concave function.}, a closed form for the solution can be found by imposing: $$\frac{\partial{}}{\partial{p_i}}\frac{1}{S} \sum_{j=1}^{S}\mathcal{I}_{\{\mathcal{O}(\mathbf{U}(\mathbf{z}_j))\leq \gamma\}} \:\mbox{ln}(g(\mathbf{z}_j,\mathbf{p}))=0,$$ leading to: 


\begin{equation} 
%  \frac{\partial{}}{\partial{p_i}}\frac{1}{S} \sum_{j=1}^{S}\mathcal{I}_{\{\mathcal{O}(\mathbf{U}(\mathbf{z}_j))\leq \gamma\}} \:\mbox{ln}(g(\mathbf{z}_j,\mathbf{p}))=0 \rightarrow \\
% \nonumber
% \frac{1}{(1-p_i)p_i} \sum_{j=1}^{S}\mathcal{I}_{\{\mathcal{O}(\mathbf{U}(\mathbf{z_j}))\leq \gamma\}}(z_{ij}-p_i)=0 \rightarrow \\
p_i=\frac{\sum_{j=1}^{S}\mathcal{I}_{\{\mathcal{O}(\mathbf{U}(\mathbf{z}_j))\leq \gamma\}}z_{ij}}{\sum_{j=1}^{S}\mathcal{I}_{\{\mathcal{O}(\mathbf{U}(\mathbf{z}_j))\leq \gamma\}}}\:\;\: i=1 \cdots m;
\label{closed form solution}
\end{equation}

In the practical use, the result in the equation (\ref{closed form solution}) is used for updating the distribution $\mathbf{p}$ as follows:

\begin{equation}
\label{closed form solution2}
p_i=(1-\alpha)p_i+\alpha \frac{\sum_{j=1}^{S}\mathcal{I}_{\{\mathcal{O}(\mathbf{U}(\mathbf{z}_j))\leq \gamma\}}z_{ij}}{\sum_{j=1}^{S}\mathcal{I}_{\{\mathcal{O}(\mathbf{U}(\mathbf{z}_j))\leq \gamma\}}} .
\end{equation}

%where at its entries closer to $1$ correspond the entries of $\mathbf{z}$ with value $1$.

The mathematical analysis about the choice of the parameter $\alpha$ is provided in the Appendix of this work. Further, indications on the choice of $\alpha$ can be found in \cite{rubinstein04,Costa2007, Wu2014}.
The derivation of equations (\ref{parameter estimation}-\ref{closed form solution}), as well as, the optimality of $g(\mathbf{z}_j,\mathbf{p})$ is  proven in \cite{rubinstein04}.

%Summarizing, we found the density distribution of the entries in $\mathbf{z}$ that take $1$-value: these entities provide the set of the indexes of the features that minimize the objective function $\mathcal{O}(\mathbf{U}(\mathbf{z}))$ that is the conditional entropy  $\mathbf{H}( \mathbf{y}| \mathbf{U}) .

The solution of the problem defined in (\ref{parameter estimation}) is achieved through Algorithm \ref{algo:main_CE}.

\begin{algorithm} [ht]
\caption{CE-based algorithm for FS}
\label{algo:main_CE}
\begin{algorithmic}[1]
\Procedure{CE}{$\mathbf{X},\mathbf{y},\mathbf{p}^G$}
\State $\mathbf{p}^l\gets\mathbf{p}^G$
\State $\mathbf{Z}\gets$generateRandomSample$(S,\mathbf{p}^l)$
% \Comment{$\mathbf{Z}\in\{0,1\}^{S\times m}$}
\State $\mathbf{u}\gets \{\}$
\ForAll{$\mathbf{z}\in\mathbf{Z}$}
\State $\mathbf{U} \gets$ getSubset($\mathbf{X}$,$\mathbf{z}$)
% \Comment{$\mathbf{U}\in\{0,1\}^{n\times \sum_{i=1}^S \mathcal{I}_{\{\mathbf{z}_i=1\}}}$}
\State $\mathbf{u}\gets\mathbf{u}\cup \mathbf{H}(\mathbf{y}|\mathbf{U})$
\EndFor
\State $\gamma \gets$ computePercentile($\mathbf{u},1-\beta$)
\State updateProbabilties($\mathbf{p}^l$,$\mathbf{u},\gamma$)
\Comment{Eq. (\ref{closed form solution2}) }
\State \Return $\mathbf{p}^l$
\EndProcedure
\end{algorithmic}
\end{algorithm}
%%========================================================================================
%%========================================================================================

\section{Federated Feature Selection}
\label{sec:fed_approach}
In this section we present how we exploit the cross-entropy based feature selection algorithm presented in Section \ref{sec:FE_theory_MAIN} and summarised in Algorithm \ref{algo:main_CE} to design our distributed and federated feature selection algorithm \ac{FFS}, described in Algorithms \ref{algo:federated_algo_server} and \ref{algo:federated_algo_client}. They cover, respectively, the two functional blocks of \ac{FFS}, i.e., Algorithm \ref{algo:federated_algo_server} is executed by the \ac{ES}  to coordinate the distributed feature selection and Algorithm \ref{algo:federated_algo_client} runs on the clients. The \ac{FFS} is an iterative procedure. At the beginning, the \ac{ES} sends to the clients involved in the process a vector $\mathbf{p^{G}} \in \mathbb{R}^d$ where each element represents the probability that each feature has to be selected according to its importance (lines 8-10 of Alg.\ref{algo:federated_algo_server}). Each element of $\mathbf{p}^G$ is initialized to $0.5$, i.e., this is a common choice when using the CE algorithm. The vector $\mathbf{p}^G$ represents a piece of global information that the \ac{ES} shares with the client nodes.  Each client $l$ uses it to initialize its local copy of the probability vector $\mathbf{p}^{l}$ and runs the local feature selection procedure based on its local data (lines 2-3 of Alg. \ref{algo:federated_algo_client}). At the end of the local feature selection, the $l$-th client sends to the \ac{ES} the locally updated features' probability vector  $\mathbf{p_{new}^l}$ and a control information regarding the cardinality of its local data $n^{l}$ whose purpose will become clear in the following. The \ac{ES} computes the new global probability vector by aggregating the ones received from the clients (line 13 of Alg. \ref{algo:federated_algo_server}). The updated vector $\mathbf{p}_{r+1}^G$ is transmitted to the nodes that, once received, they run Algorithm \ref{algo:federated_algo_client} initializing the local probability vector with the new global one. This procedure iterates until the distribution global probability vector converges to a stable one. In \ac{FFS} we check convergence by comparing the distribution of the current global probability vector $\mathbf{p}_r^{G}$ to the previous one $\mathbf{p}_{old}^G$ using the Kolmogov-Smirnov statistical test for two one-dimensional samples (KS-test). The procedure stops when (i) the p-value of the KS-test is greater than a fixed threshold ($\tau_1=0.995$)\footnote{We empirically observed that the closer $\tau_1$ to one, the more accurate the solution.} and, (ii) its variation from one update to the other is negligible, i.e., $\tau_2 = 10^{-6}$ (line 7 of Alg. \ref{algo:federated_algo_server}).

The core point of Algorithm \ref{algo:federated_algo_server} regards the aggregation step (line 13 al Alg. \ref{algo:federated_algo_server}) where the \ac{ES} merges the local probability vectors into the global one, which, in our solution it is defined as a weighted average.
Formally, we assume that each node acquires a number of \textit{i.i.d.} records $n^{l}$  to perform \ac{FS}, and that the nodes share the same set of features $\mathbf{X}$.
%, where $n_i \neq n_j$ $\forall \; i \neq j $ with $i,j\in\{1, \dots, L\}$, but all the records are identically distributed. 
The global probability $\mathbf{p}^{\mathbf{G}}$ used for the \ac{FS} can be written as follows:
\begin{equation}
\label{eq:joint_probability}
    \mathbf{p}^{G}=\sum_l \mathbf{p}^{l} q^{l},
\end{equation}
 where $\mathbf{p}^{(l)}$ is the solution of problem (\ref{parameter estimation}) at node $l$ obtained \replaced[id=PC]{by using}{using} Algorithm \ref{algo:main_CE},
 and $q^{(l)}$, whose formal definition is provided in equation (\ref{eq:probability_data_from_node}) weights the probability vector of node $l$ \textit{w.r.t.} the other nodes. 

\begin{equation}
    \label{eq:probability_data_from_node}
    q^{l}=\frac{n^{l}}{\displaystyle\sum_l n^{l}}
\end{equation}

According to equation (\ref{eq:probability_data_from_node}), we weight the probability vector $p^{l}$ of node $l$ proportionally to the size of its local dataset compared to the whole amount of data present in the system. In this way, we can contrast situations where local datasets are heterogeneous w.r.t. the size.

In \ac{FFS}, the updating scheme can be, at least in principle, both synchronous and asynchronous, provided that the set of nodes involved in the process does not change over time.\footnote{Note that this condition does not imply that all nodes must be active during the entire process. In fact, as we will show in Section \ref{sec:num_results} our system is robust to the presence of churning nodes.} Precisely,  we  assume  a  system  where  the  \ac{ES} expects, after  sending  the  updated  global  probability  vector  to  the nodes, to receive their local updates within a fixed time slot, after which, it begins the aggregation step  using  only  the  information  received.  Therefore, the number of updates' used to compute the new global probability vector might change because a subset of nodes could not communicate their update within the time limit imposed by the \ac{ES}. Regardless of the number of nodes that contributed to the aggregation step during one round of communication, the \ac{ES} broadcasts the new global probability vector $\bf{p}^G$ to \emph{all} nodes in the system. In this way, all nodes start the new round of local computation from the same starting point, and, consequently, we dramatically limit the potentially detrimental effects deriving from the aggregation of outdated local probability vectors. Moreover, as proved by the convergence analysis provided in the Appendix, independently from the updating scheme, \ac{FFS} converges the infinite number of steps to the very same solution that would be found running the CE-based algorithm for \ac{FS} in centralised settings i.e., with complete access to the entire dataset.

\begin{algorithm} [ht]
\caption{Server side Federated Feature Selection algorithm}
\label{algo:federated_algo_server}
\begin{algorithmic}[1]
\Procedure{Server-Node}{}
% \State $v_{old} \gets 0$
\State $v \gets 0$
\Comment{p-value of Kolmogorov-Smirnov test}
\State $\tau_1 \gets .995$
\State $\tau_2 \gets 10^{-6}$
\Comment{Thresholds to check convergence}
\State $r \gets 0$
\Comment{$r$-th communication round}
\State $\mathbf{p}^{\mathbf{G}}_{r} \gets \{1/2\;|\;\forall\; p_{i}\;  i=1,\dots,m\}$
% \State CONVERGED $\gets$ \textit{False}
\While{$v \geq \tau_1 \land |v-v_{old}| \leq \tau_2$}
\Comment{repeat until convergence is met}
\ForAll {$l\in L$}
\State sendUpdateToClient($l,\mathbf{p}^{G}_{r}$)
\EndFor
\State receiveLocalUpdateFromNodes($\mathbf{p}^{(l)}_{new},n^{(l)}$)
\State $\mathbf{p}^{G}_{old} \gets \mathbf{p}^{G}_{r}$
\State $\mathbf{p}^{G}_{r} \gets$ updateGlobalProbability()
\Comment{Eq. (\ref{eq:joint_probability})}
\State $v_{old} \gets v$
\State $v \gets $KolmogorovSmirnovTest$(\mathbf{p}^{G}_{old},\mathbf{p}^{G}_{r})$
% \If {$v \geq \tau_1 \land |v-v_{old}| \leq \tau_2$}
% \State CONVERGED $\gets$ \textit{True}
% \EndIf
\State $r \gets r+1$

\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm} [ht]
\caption{Client side Federated Feature Selection algorithm}
\label{algo:federated_algo_client}
\begin{algorithmic}[1]
\Procedure{Client-Node}{}
% \State $t \leftarrow 0$
\State $\mathbf{p}^l \gets$ receiveFromServer($\mathbf{p}_r^G$)
\State $\mathbf{p}_{new}^l \gets$ CE($\mathbf{X}^l,\mathbf{y}^l,\mathbf{p}^l$)
\Comment{Algorithm \ref{algo:main_CE}}
\State sendToServer($\mathbf{p}_{new}^l, n^l$)
\EndProcedure
\end{algorithmic}
\end{algorithm}


